Exploiting all phone media? A multidimensional network analysis of phone users' sociality

The growing awareness that human communications and social interactions are assuming a stratified structure, due to the availability of multiple techno-communication channels, including online social networks, mobile phone calls, short messages (SMS) and e-mails, has recently led to the study of multidimensional networks, as a step further the classical Social Network Analysis. A few papers have been dedicated to develop the theoretical framework to deal with such multiplex networks and to analyze some example of multidimensional social networks. In this context we perform the first study of the multiplex mobile social network, gathered from the records of both call and text message activities of millions of users of a large mobile phone operator over a period of 12 weeks. While social networks constructed from mobile phone datasets have drawn great attention in recent years, so far studies have dealt with text message and call data, separately, providing a very partial view of people sociality expressed on phone. Here we analyze how the call and the text message dimensions overlap showing how many information about links and nodes could be lost only accounting for a single layer and how users adopt different media channels to interact with their neighborhood.

==> Multireciprocity.tex <==
\section{Multireciprocity in mobile phone data}\label{sec:Multireciprocity}

\begin{figure*}[t]
\centering
\begin{subfigure}{0.70\textwidth}
\includegraphics[width=\textwidth]{images/multireciprocityClassesSchema.pdf}
\caption{}
\label{fig:multireciprocityClasses}
\end{subfigure}
%\begin{subfigure}{0.28\textwidth}
%\includegraphics[width=\textwidth]{images/multireciprocityClassesSchema.pdf}
%\caption{}
%\label{fig:otherFigure}
%\end{subfigure}
\caption{TO DO}
\label{fig:multireciprocity}
\end{figure*}

The communication chance offered by any telecommunication carrier allows users to maintain or establish their social relationships leveraging different media. For instance a group of friends could prefer the SMS channel to organize the fun of their night, while for a more intimate and rich interaction they prefer to call. This way a mutual communication and connection could be establish interleaving the different media channel. Consequently we need to extend a basic concept which characterizes the tendency of user to establish mutual relationship, {\em i.e.} the reciprocity or mutuality. \textbf{Importanza della reciprocity in altre OSN}.
Specifically, in this paper, we take into account the dyad census extending the approach presented in Wassermann and Faust. In fact we are more interesting in how a specific pair of users (dyad)   

%\par A further step in understanding the nature of social interactions in the mobile phone dataset, we focus on a specific correlation typical of the directed networks: the link reciprocity, \textit{i.e.} the tendency of node pairs to establish mutual connections. In evaluating the link reciprocity we follow the approach presented in \cite{Garlaschelli04} which overcome the classical definition introducing the correlation coefficient $\rho$ between the entries of the adjacency matrix of a directed graph:
%\begin{equation}
%\rho=\frac{\sum_{i\neq j}(a_{ij}-d)(a_{ji}-d)}{\sum_{i\neq j}(a_{ij}-d)^{2}} = \frac{r-d}{1-d}
%\end{equation}
%where $r$ is the common definition of reciprocity and $d$ is the density of the graph. The correlation coefficient $\rho$ is an absolute quantity which directly allows to distinguish between reciprocal ($\rho>0$) and antireciprocal ($\rho<0$) networks, with mutual links occurring more and less often than random respectively and to order different networks with respect to their actual degree of reciprocity. We compute the reciprocity $\rho$ on $G_{c}$ and $G_{s}$ obtaining the respective values $\rho_{c}=0.44$ and $\rho_{s}=0.57$. These results that $G_{c}$ and $G_{s}$ are quite reciprocal as well as the relative social interactions, furthermore we can insert the two graphs in the reciprocity class characterizing also the World Wide Web.
\par The previous definitions of reciprocity, even the simplest one, are not suitable for directed multigraph is they do not consider the presence of multiple links between a pair of nodes. To overcome the limitation we extended the simple definition of reciprocity to the multigraph case:
\begin{definition}
Let $G_{cs}$ a multigraph, the link reciprocity $r$ is defined as 
%$|E^{\rightleftarrow}_{cs}|/|E_{cs}|$ where $E^{\rightleftarrow}_{cs}$ %
$|E^{cs}|/|E_{cs}|$ where $E_{cs}$ 
is the number of links pointing in both directions with respect to a label
\end{definition}
The computation of the mutual direction w.r.t a label avoids to consider as mutual links that lay on different layers as depicted in the \figurename\ref{fig:multireciprocity} where the links $(i,j,sms)$ and $(j,i,call)$ can not be considered mutual because have different labels. The computed reciprocity $r$ on $G_{cs}$ is in accordance with the ones calculated on $G_{c}$ and $G_{s}$ and is equals to $0.43$. thus the multigraph $G_{cs}$ is reciprocal as the corresponding call and SMS graphs.
